Data-Efficient Mutual Information Neural Estimator

Measuring Mutual Information (MI) between high-dimensional, continuous, random variables from observed samples has wide theoretical and practical applications. Recent work, MINE (Belghazi et al. 2018), focused on estimating tight variational lower bounds of MI using neural networks, but assumed unlimited supply of samples to prevent overfitting. In real world applications, data is not always available at a surplus. In this work, we focus on improving data efficiency and propose a Data-Efficient MINE Estimator (DEMINE), by developing a relaxed predictive MI lower bound that can be estimated at higher data efficiency by orders of magnitudes. The predictive MI lower bound also enables us to develop a new meta-learning approach using task augmentation, Meta-DEMINE, to improve generalization of the network and further boost estimation accuracy empirically. With improved data-efficiency, our estimators enables statistical testing of dependency at practical dataset sizes. We demonstrate the effectiveness of our estimators on synthetic benchmarks and a real world fMRI data, with application of inter-subject correlation analysis.

==> ch/_OLD_00-Abstract.tex <==
\begin{abstract}
Measuring Mutual Information (MI) between high-dimensional, continuous, random variables from observed samples has wide theoretical and practical applications. Traditional MI estimators, such as \cite{Kraskov2004}, are capable of capturing MI between low-dimensional signals, but fall short when the dimensionality increases. Existing neural estimators, such as \cite{MINE}, searches for a $d$-dimensional neural network that maximizes a variational lower bound for mutual information estimation; however, this requires $O(d\log d)$ observed samples to prevent from overfitting. For practical mutual information estimation in real world applications, data is not always available at a surplus, especially in cases where acquisition of the data is prohibitively expensive, as in fMRI data analysis. 

We introduce a scalable, data-efficient MI estimator. By coupling a learning-based view of the MI lower bound with meta-learning, \metaalgo achieves high-confidence estimations irrespective of network size and with improved accuracy at practical dataset sizes. We demonstrate the effectiveness of \metaalgo on synthetic benchmarks as well as a real world application of fMRI inter-subject correlation analysis.
%Humans use language to effectively transmit brain representations among conspecifics. The efficacy of this transmission, in terms of listener comprehension, is predicted by speaker–listener neural synchrony and synchrony among listeners. To date, most work has measured brain-to-brain synchrony using inter-subject correlation (ISC); quantified as the Pearson product-moment correlation coefficient between response time series for corresponding voxels or regions of interest (ROIs) across individuals. By modeling each subject's neural responses using the responses of other subjects, ISC analyses provide novel insights. However, Pearson correlation only captures the linear association between voxel-wise response time series across subjects. In this work, inspired by recent successes in mutual information estimation in machine learning, we propose a new measure that utilizes neural networks, Neural Mutual Information (\basealgo), to capture more complex signatures of brain-to-brain coupling. \basealgo captures distributed, nonlinear inter-subject coupling by learning to predict the lower bound of mutual information between spatio-temporal functional Magnetic Resonance Imaging (fMRI) responses across individuals. Our approach diverges from by training a neural network to predict mutual information on a seen dataset and estimate if on an unseen dataset which avoids overfitting and applicable to small datasets. In brief, by using neural networks to encode continuous fMRI responses, we can learn nonlinear and higher-order inter-subject associations.
\end{abstract}

==> ch/_OLD_01-Intro.tex <==
\section{Introduction}
Mutual Information (MI) is an important, theoretically grounded, measures of similarity between random variables. MI captures general non-linear statistical dependencies between random variables. It is widely used quantity in various machine learning tasks ranging from classification to feature selection and neural network analysis. 



%Traditional approaches used binning \cite{BinningOld,BinningNew}, entropy estimation from k-nearest neighbor distances~\cite{Kraskov2004} making them data efficient, adaptive with minimal bias, however, when it came to large dimensionality these methods fail to scale. In high dimensional, continuous spaces, such as text, images, videos, fMRI and other time-series signals, measuring MI between random variables is prohibitively expensive and complex computation. 

%With the success of neural networks capturing similarity in representations and distributions of large dimensional spaces, a new Mutual Information Neural Estimator (MINE) was proposed~\cite{MINE}. 
%Similar to Generative Adversarial Networks (GANs) \cite{Goodfellow17} estimating an implicit density using Kullback-Leibler (KL) divergence without any assumptions about the distributions, MINE uses KL-divergence, and cast the estimation in the same framework as $f-$divergences using a dual formulation \cite{Nguyen_2010}. 
%Compared to traditional methods, MINE is scalable, flexible and optimized using back-propagation. 

In this work, inspired by recent successes of~\cite{MINE}, we propose a new measure that utilizes neural networks, Data Efficient Mutual Information Neural Estimator (\basealgo). Our approach diverges from~\cite{MINE} by training a neural network to predict MI on a seen dataset and estimate if on an unseen dataset which avoids overfitting and is applicable to high dimensional datasets, with small number of instances. We validate and apply \basealgo to more complex problem, that of capturing brain-to-brain coupling in functional Magnetic Resonance Imaging (fMRI) data. \basealgo captures distributed, nonlinear inter-subject coupling by learning to predict the lower bound of MI between spatio-temporal fMRI responses across individuals. In brief, by using neural networks to encode continuous fMRI responses, we can learn nonlinear and higher-order inter-subject associations.

With the success of Meta-Learning \cite{MAML}, in improve the generalization capability model by learning better hyperparameters, network architectures, initialization, and loss functions. We develop a new meta-learning framework for MI estimation, \metaalgo. We developed a task augmentation approach by utilizing MI's invariance to invertible transformations which makes meta-learning less prone to overfitting. Our contributions are summarized as follows: 1) Data Efficient Mutual Information Neural Estimator (\basealgo); 2) New formulation of meta learning using Task Augmentation (\metaalgo); 3) Application to real life, data scarse, application (fMRI).
%
%We relate these nonlinear intersubject associations to conventional ISCs, and explore how the learned associations relate to behavioral metrics of listener comprehension \todo{Fix this}.
 %
%Humans use language to effectively transmit brain representations among conspecifics. For example, after witnessing an event in the world, a speaker may use verbal communication to evoke neural representations reflecting that event in a listener's brain \cite{Hasson_CogSci2012}. The efficacy of this transmission, in terms of listener comprehension, is predicted by speaker–listener neural synchrony and synchrony among listeners \cite{stephens2010speaker}. To date, most work has measured brain-to-brain synchrony using inter-subject correlation (ISC); quantified as the Pearson product-moment correlation coefficient between response time series for corresponding voxels or regions of interest (ROIs) across individuals \cite{hasson2004intersubject}. By modeling each subject's neural responses using the responses of other subjects, ISC analyses provide novel insights. Unlike traditional fMRI analysis, which often rely on highly-controlled stimuli and trial averaging, ISC analyses are particularly well-suited to continuous, naturalistic paradigms, as they do not require an explicit model of the stimulus and are sensitive to evolving narrative context \cite{hasson2010reliability, ben2012loss}. However, Pearson correlation only captures the linear association between voxel-wise response time series across subjects. Although extensions of ISC analysis have used Granger causality \cite{schippers2010mapping} and dynamic time warping \cite{silbert2014coupled} to accommodate temporal asynchrony, it is not clear how best to circumvent these limitations. 

==> ch/_OLD_05.1-Experiment.tex <==
\section{Synthetic Evaluations}
In this section, we evaluate our approaches \basealgo and \metaalgo against baselines and state-of-the-art approaches on synthetic datasets, First, in\secref{sec:synthdata}, we describe the different datasets. Then, in \secref{sec:expsetup}, we specify the approaches evaluated. Finally, in \secref{sec:synthresults} we present our experiments results.
%
\subsection{Synthetic Datasets}\label{sec:synthdata}
%We conduct evaluations on synthetic benchmarks focusing on confidence interval and bound tightness. 
%We conduct experiments on two types of data:
%
\noindent\textbf{Multivariate Gaussian:} Following~\cite{MINE}, we define two $k$-dimensional multivariate Gaussian random variables $X$ and $Z$ which have component-wise correlation $corr(X_i,Z_j)=\delta_{ij}\rho$, where $\rho \in (-1,1)$ and $\delta_{ij}$ is Kronecker's delta. Mutual information $I(X;Z)$ has a closed form solution $I(X;Z)=-k\ln(1-\rho^2)$. We vary the parameter $\rho \in \{0,0.1,0.3,0.5,0.7\}$ and $\rho \in \{0.05,0.1,0.15,0.2,0.25\}$ for $k=1$ and $k=10$ respectively. We also vary number of samples $n \in \{ 200, 600, 2000, 6000 \}$. For each setting, we generate 10 datasets using 10 different random seeds.

\noindent\textbf{Noisy sine wave regression:} We define two random variables $X$ and $Z$, where $Z=\sin (aX)+0.05\epsilon$, $X \sim \mathcal{U}(-1,1)$ and $\epsilon \sim \mathcal{N}(0,1)$. Estimating mutual information accurately given few pairs of $(X,Z)$ requires the ability to extrapolate the sine wave given few examples. We vary the parameter $a\in \{ 20,30 \}$ to generate sine waves of different frequencies. We also vary the number of samples $n \in \{ 800,2000\}$. As a closed-form mutual information solution does not exist, we run the MI-Kraskov \cite{Kraskov2004} mutual information estimator on $1,000,000$ samples drawn from the sine wave as an estimation of ground truth. Same as multivariate Gaussian, we generate 10 datasets for each setting using 10 random seeds.
%
\subsection{Experiment Setup}\label{sec:expsetup}
%
\begin{figure}
  \centering
  \includegraphics[width=0.5\linewidth]{images/arch_synthetic.pdf}
  \caption{Network architecture used for synthetic experiments. Incoming samples of random variables $X$ and $Z$ are encoded using MLP and are combined using cosine distance followed by a scaling layer.}
  \label{fig:arch_synthetic}
\end{figure}
%
%
In our experiments we compare the following approaches:

\noindent\textbf{\basealgo}: Our base algorithm for estimating mutual information lower bound introduced in \secref{sec:Estimator}. We split the samples $(x,z)$ into 50\%-50\% as $(x,z)_{\text{train}}$ and $(x,z)_{\text{val}}$. We use a multi-layer perceptron (MLP) network with cosine distance on top for $T_\theta (X,Z)$ shown in Figure.~\ref{fig:arch_synthetic}. $X$ and $Z$ are each encoded using an MLP into embeddings.  Cosine similarity is used to join the embeddings, followed by a scaling function $M\tanh(wx+b)$ to control the bound in $[-M,M]$, where we fix $M=3$. We select the MLP hyper-parameters -- hidden size $h \in \{ 32,64,256\}$ and number of layers $\in \{ 2,3,4\}$, learning rate $l \eta \in \{ 10^{-4},3\times 10^{-4},10^{-3},3\times 10^{-3},10^{-2},3\times 10^{-2},10^{-1}\}$ and number of iterations $N \in \{ 5,10,20,50,100,200,500,1000,2000\}$ -- through a grid search using 4-fold cross-validation on $(x,z)_{\text{train}}$.

\noindent\textbf{\metaalgo}: Our meta learning algorithm for estimating mutual information lower bound introduced in \secref{sec:Meta}. We use the same  50\%-50\% split of the data into $(x,z)_{\text{train}}$ and $(x,z)_{\text{val}}$. The model architecture and hyper parameters as specified in \basealgo, with additional optimization-related hyper parameters fixed to $N_M=5,000$, $N_T=3$, $\eta_{\text{meta}}=3\times 10^{-3}$, ratio $r=0.8$ for faster optimization. PEPG~\cite{pepg} is used for computing gradient for meta-optimization due to the large $N_O$.

\noindent\textbf{\textit{MINE-f-ES}}\footnote{As we focus on mutual information estimation performance using few samples, optimizing \textit{MINE} to convergence will result in overfitting and \textit{MINE} will almost always incorrectly report $\reallywidehat{I(X,Z)}_n=M$ which will not make a meaningful comparison.}: \textit{Mine-f} with early stopping, the \textit{MINE} mutual information lower bound estimator~\cite{MINE} introduced in \secref{sec:Background}, but augmented with early stopping to reduce overfitting. We use \textit{MINE-f} and stop optimization before $T_\theta(X,Z)$ overfits, by selecting hyperparameters using the same cross validation protocol as \basealgo, and compute \textit{MINE-f-ES}. \textit{MINE-f} with early stopping receives the entire set of samples $(x,z)$ and use the same model architecture as \basealgo.

\noindent\textbf{MI-Kraskov}: The KSG estimator~\cite{Kraskov2004}, a $k$-NN-based non-parametric mutual information estimator. We use publicly available implementations\footnote{Scikit-learn for 1-D random variables: \url{https://scikit-learn.org/stable/modules/generated/sklearn.feature_selection.mutual_info_classif.html} where estimator outputs are thresholded to be non-negative. Implementation by \cite{Gao2017} for high-dimensional random variables \url{https://github.com/wgao9/knnie}.}, which computes mutual information between high-dimensional random variable $X$ and one-dimensional random variable $Z$. We use the entire set of samples $(x,z)$ and the default hyper parameter $\text{n\_neighbors}=3$.
%
\subsection{Result}\label{sec:synthresults}
%
Mutual estimation results for all the 1-Dimensional (1D) Gaussian, 10-dimensional (10D) Gaussian and sine wave datasets are available in Figure~\ref{fig:1d_gaussian}, \ref{fig:10d_gaussian} and \ref{fig:sine_wave} respectively. For each dataset we run each algorithm on datasets generated using 10 different seeds. We report 95\% confidence intervals of \basealgo and \metaalgo lower bound based on (\ref{eqn:samplecomplexity}). We report confidence intervals of \textit{MINE-f-ES} lower bound based on  (\ref{eqn:MINEsamples}), in which $d$ and $K$ are computed from $\theta$ while assuming $L=1$. MI-Kraskov mutual information estimator, however, does not come with analytical bound guarantees. The numerical values of the mean values over 10 runs and the confidence intervals are reported in Tables \ref{table:1D_gaussian}, \ref{table:10D_gaussian} and \ref{table:sine_wave}.

\noindent\textbf{The 1D Gaussian results:} results in Figure~\ref{fig:1d_gaussian} serves as a consistency check. Both \basealgo and \metaalgo are able to reliably estimate mutual information bounds for all $\rho$s given $n \ge 300$ samples.  Notably, for 1D Gaussian $\rho=0.0$ (Figure~\ref{fig:1d_gaussian} first row), MI-Kraskov and \textit{MINE-f-ES} both constantly predict positive values yet the true mutual information is 0, even at 1,000 samples when 1,000 points have been sampled between $X\in \mathcal{U}(-1,1)$. We find that in general, \textit{MINE-f-ES} and MI-Kraskov tend to produce aggressive mutual information estimates, which often seems to be closer to the true mutual information values, yet are not justified and with extremely loose confidence intervals. Given a positive detection yet with a low confidence, it would be impossible to conclude if $X$ and $Z$ are statistically dependent or not. \basealgo and \metaalgo produce lower bound estimations with tighter confidence intervals. For 1D Gaussian $\rho=0.0$, lower bound estimations by \basealgo and \metaalgo are mostly negative, with 95\% confidence intervals consistent with the null hypothesis $I(X;Z)=0$. For 1D Gaussian $\rho=0.5$ (Figure~\ref{fig:1d_gaussian} fifth row) $n=2000$, \basealgo and \metaalgo signals statistically significant dependency.

\noindent\textbf{The 10D Gaussian results:} results in Figure~\ref{fig:10d_gaussian} tests the performance of MI estimation for high-dimensional random variables. The gap between the estimations and the ground truth MI becomes visibly larger than the 1D Gaussian case, which demonstrates the challenge of MI estimation with few samples in high-dimensional space. \textit{MINE-f-ES} produces lower bound estimations closest to the ground truth MI yet are low confidence and overshoot on few samples. \basealgo provides high-confidence estimations close to the ground truth, and \metaalgo slightly but consistently improves the estimations of \basealgo. MI-Kraskov on the other hand, provides estimations far from ground truth.

\noindent\textbf{Sine wave results:} The effect of meta learning is most significant for sine wave result shown in Figure~\ref{fig:sine_wave}. Despite delivering good performance for 1D Gaussians, MI-Kraskov significantly under estimates the amount of mutual information available in the 1D sine waves. \basealgo detects significant dependency in the 2000 sample cases. By incorporating MAML which have been shown to learn the structure of sine waves, \metaalgo significantly improves mutual information estimation results and are even able to detect significant dependency in the $a=20$ 400 samples case. 

To study the effect of task augmentation, we compare the performance of \metaalgo with and without task augmentation for 10D Gaussian $\rho=0.2$ using 6000 samples. Figure~\ref{fig:task_aug} shows the progression of the MI estimation (left) as well as the inverse trainloss (right) over the course of training. Indeed, maximizing cross-validation performance without task augmentation results in rapid overfitting and very little performance gain. With task augmentation on, the inverse trainloss reduces due to the difficulty of performing all the augmented tasks. The MI estimation, however, shows no overfitting in 2500 iterations with performance keep increasing to beyond \basealgo through the course of training.
%
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/1D_rho0.0.png} \\
  \includegraphics[width=\linewidth]{images/1D_rho0.1.png} \\ 
  \includegraphics[width=\linewidth]{images/1D_rho0.3.png} \\
  \includegraphics[width=\linewidth]{images/1D_rho0.5.png} \\
  \includegraphics[width=\linewidth]{images/1D_rho0.7.png}
  \caption{1D Gaussian results for MI-Kraskov, \textit{MINE-f} with early stopping (MINE-f ES), \basealgo and \metaalgo on 1D correlated Gaussian random variables with correlation $\rho \in \{0.0,0.1,0.3,0.5,0.7\}$ (top to bottom) and number of samples $n\in \{200,600,2000 \}$ (left to right). Results of 10 runs with confidence intervals are recorded and visualized. Ground truth MI is visualized as the horizontal line. MI-Kraskov and MINE-f ES makes aggressive yet low confidence estimations which can be seen in the $\rho=0.0$ case. \basealgo and \metaalgo detects statistically significant dependency for $\rho=0.5$ and $\rho=0.7$.}
  \label{fig:1d_gaussian}
\end{figure}
%
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/10D_rho0.05.png} \\ \includegraphics[width=\linewidth]{images/10D_rho0.10.png} \\  \includegraphics[width=\linewidth]{images/10D_rho0.15.png} \\
  \includegraphics[width=\linewidth]{images/10D_rho0.20.png} \\
  \includegraphics[width=\linewidth]{images/10D_rho0.25.png}
  \caption{10D Gaussian results for MI-Kraskov, \textit{MINE-f} with early stopping (MINE-f ES), \basealgo and \metaalgo on 10D diagonally correlated Gaussian random variables with correlation $\rho \in \{0.05,0.10,0.15,0.20,0.25\}$ (top to bottom) and number of samples $n\in \{200,600,2000,6000 \}$ (left to right). Results of 10 runs with confidence intervals are recorded and visualized. Ground truth MI is visualized as the horizontal line. MINE-f ES makes aggressive yet low confidence estimations which can be seen in the $\rho=0.05$ case. MI-Kraskov under estimates mutual information. \basealgo and \metaalgo detects statistically significant dependency for $\rho=0.15,0.20,0.25$.}
  \label{fig:10d_gaussian}
\end{figure}
%
\input{images/All_Gaussians_combined.tex}
%
\input{images/sine_wave.tex}
%
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/sine_wave_rho20.png}\\ \includegraphics[width=\linewidth]{images/sine_wave_rho30.png} 
  \caption{Sine wave results for MI-Kraskov, \textit{MINE-f} with early stopping (MINE-f ES), \basealgo and \metaalgo on 1D random variables (X,Y) where $Y=sin(aX)$. $a \in \{20,30\}$ (top to bottom) and number of samples $n\in \{800,2000\}$ (left to right). Results of 10 runs with confidence intervals are recorded and visualized. Estimated MI from $1,000,000$ samples is visualized as the horizontal dashed line. MINE-f ES makes aggressive yet low confidence estimations. MI-Kraskov under estimates mutual information. \basealgo and \metaalgo detects statistically significant dependency for both datasets. \metaalgo shows significant accuracy improvements over \basealgo.}
  \label{fig:sine_wave}
\end{figure}
%
%\todo{Figure x} compares the $T_{\tilde{\theta}}(X,Z)$ learned by \basealgo and \metaalgo. \metaalgo outside of $X \in (-1,1)$ still shows the sine wave shape, despite that no training data outside of $X \in (-1,1)$ was provided. Where as \basealgo shows smoothing but limited generalization. Note that different from experiments presented in MAML~\cite{MAML} which uses unlimited training data but focus on extreme few-shot sine wave regression, our \metaalgo uses a fixed number of samples from a single sine wave and focus on improvements in data-efficiency.
%
\begin{figure}
  \centering
  \includegraphics[width=0.7\linewidth]{images/task_augmentation.pdf}
  \caption{Validation MI estimation and trainloss progress of running \metaalgo with and without task augmentation on 10D Gaussian $\rho=0.20$, $n=6000$ over 2500 iterations. Without task augmentation, \metaalgo quickly overfits and shows only small improvements on top of \basealgo. Task augmentation reduces overfitting as well as greatly improves mutual information estimation results. }
  \label{fig:task_aug}
\end{figure}

==> ch/_OLD_05.2-fMRI.tex <==
\section{Application: fMRI Inter-subject correlation (ISC) analysis}

To demonstrate application of \basealgo and \metaalgo on real data, we study the effectiveness of using \basealgo and \metaalgo for Inter-subject Correlation (ISC) analysis of fMRI images.

Humans use language to effectively transmit brain representations among conspecifics. For example, after witnessing an event in the world, a speaker may use verbal communication to evoke neural representations reflecting that event in a listener's brain \cite{Hasson_CogSci2012}. The efficacy of this transmission, in terms of listener comprehension, is predicted by speaker–listener neural synchrony and synchrony among listeners \cite{stephens2010speaker}. To date, most work has measured brain-to-brain synchrony using inter-subject correlation (ISC); quantified as the Pearson product-moment correlation coefficient between response time series for corresponding voxels or regions of interest (ROIs) across individuals \cite{hasson2004intersubject}. By modeling each subject's neural responses using the responses of other subjects, ISC analyses provide novel insights. Unlike traditional fMRI analysis, which often rely on highly-controlled stimuli and trial averaging, ISC analyses are particularly well-suited to continuous, naturalistic paradigms, as they do not require an explicit model of the stimulus and are sensitive to evolving narrative context \cite{hasson2010reliability, ben2012loss}. 
However, Pearson correlation only captures the linear association between voxel-wise response time series across subjects. 
Although extensions of ISC analysis have used Granger causality \cite{schippers2010mapping} and dynamic time warping \cite{silbert2014coupled} to accommodate temporal asynchrony, it is not clear how best to circumvent these limitations.
In this work, inspired by recent successes in mutual information estimation in machine learning\cite{MINE}, we propose data-efficient \basealgo and \metaalgo for capturing more complex signatures of brain-to-brain coupling by using neural networks to encode continuous fMRI responses, we can learn nonlinear and higher-order inter-subject associations.

\subsection{Dataset and Metrics}
\textbf{New fMRI Dataset.} We apply the proposed model to a newly collected fMRI dataset with 40 participants (mean age = 23.3 years, SD = 8.9, range: 18–53; 27 female) listening to four spoken stories\footnote{Two of the stories were told by a professional storyteller undergoing an fMRI scan; however, fMRI data for the speaker were not analyzed for the present work due to the head motion induced by speech production.}\footnote{The study was conducted in compliance with the Institutional Review Board of the University}. The stories were renditions of “Pie Man” and “Running from the Bronx” by Jim O’Grady \cite{PieMan, Bronx}, “The Man Who Forgot Ray Bradbury” by Neil Gaiman \cite{Forgot}, and “I Knew You Were Black” by Carol Daniel \cite{Black}; story durations were ~7, 9, 14, and 13 minutes, respectively. After scanning, participants completed a questionnaire comprising 25–30 questions per story intended to measure narrative comprehension. The questionnaires included multiple choice, True/False, and fill-in-the-blank questions, as well as four additional subjective ratings per story. Functional and structural images were acquired using a 3T Siemens Prisma with a 64-channel head coil\footnote{See Appendix for additional image acquisition details.}. Briefly, functional images were acquired in an interleaved fashion using gradient-echo echo-planar imaging with a multiband acceleration factor of 3 (TR/TE = 1500/31 ms, resolution = 2.5 mm isotropic voxels, full brain coverage).
%
%In the end, we have 4 stories, each with N=40 fMRI sequences.
%
%The fMRI voxels are mapped onto a standard brain using some technique.
%
%The fMRI sequences are preprocessed into 3mm  voxels.
%
%We normalize the fMRI sequences by mean-std.
%
%We partition data by subject, where sequences from 20 subjects go into train and sequences from the other 20 subjects go into test. 
%
%We focus on the dDMN region, the ISC voxels and the gray matter region.
%
%We also investigate ISC voxels and gray matter with the auditory regions removed for analyzing synchronous non-auditory brain activities.
%
All fMRI data were formatted according to the Brain Imaging Data Structure (BIDS) standard \cite{gorgolewski2016brain} and preprocessed using fMRIPrep \cite{Esteban_2018}\footnote{See Appendix for additional preprocessing details.}. Functional data were corrected for slice timing, head motion, and susceptibility distortion, and normalized to MNI space using nonlinear registration. Nuisance variables comprising head motion parameters, framewise displacement, linear and quadratic trends, sine/cosine bases for high-pass filtering (0.007 Hz), and six principal component time series from cerebrospinal fluid (CSF) and white matter were regressed out of the signal using AFNI \cite{Cox_1996}.

The fMRI data were first partitioned into a seen set of 20 subjects and a unseen set of 20 separate subjects. We restricted our analysis to three subsets of voxels: an anatomically defined gray matter mask (GM; 22,541 voxels), as well as functionally-defined masks of high ISC voxels (ISC; 15,041 voxels) and dorsal Default-Mode Network voxels (dDMN; 3,940 voxels). All masks were defined in MNI space, and the ISC and dDMN masks were defined using independent data from previous studies \cite{simony2016dynamic}.
%The fMRI data comprise \dimension{\FMRI}{\FMRIdim}\todo{what is C here? is this necessary?}\todo{C is left over from our spacial model indicating # of channels.} for each subject, where \FMRIspaD represents the spatial dimensions of each volume and \T represents the number of samples (TRs) during auditory stimulus presentation.
The fMRI data comprise \dimension{\FMRI}{\FMRIdimFlat} for each subject, where \xV represents the flattened and masked voxel space and \T represents the number of samples (TRs) during auditory stimulus presentation.

%For each audio segment, subjects were asked to pay attention and passively listen to the story. Subjects were also instructed to attend to the details of the narrative.


\textbf{Details on Dataset Collection}
Functional and structural images were acquired using a 3T Siemens Magnetom Prisma with a 64-channel head coil. Functional, blood-oxygenation-level-dependent (BOLD) images were acquired in an interleaved fashion using gradient-echo echo-planar imaging with pre-scan normalization, fat suppression, a multiband acceleration factor of 3, and no in-plane acceleration: TR/TE = 1500/31 ms, flip angle = 67°, bandwidth = 2480 Hz/Px, resolution = 2.5 mm3 isotropic voxels, matrix size = 96 x 96, FoV = 240 x 240 mm, 48 axial slices with roughly full brain coverage and no gap, anterior–posterior phase encoding. At the beginning of each scanning session, a T1-weighted structural scan was acquired using a high-resolution single-shot MPRAGE sequence with an in-plane acceleration factor of 2 using GRAPPA: TR/TE/TI = 2530/3.3/1100 ms, flip angle = 7°, resolution = 1.0 x 1.0 x 1.0 mm voxels, matrix size = 256 x 256, FoV = 256 x 256 x 176 mm, 176 sagittal slices, ascending acquisition, anterior–posterior phase encoding, no fat suppression, 5 min 53 s total acquisition time. At the end of each scanning session a T2-weighted structural scan was acquired using the same acquisition parameters and geometry as the T1-weighted structural image: TR/TE = 3200/428 ms, 4 min 40 s total acquisition time. A field map was acquired at the beginning of each scanning session, but was not used in subsequent analyses.

\textbf{Details on Dataset Preprocessing}
Preprocessing was performed using fMRIPrep \cite{Esteban_2018}, a Nipype \cite{Gorgolewski_2011} based tool. T1-weighted images were corrected for intensity non-uniformity using N4 bias field correction \cite{Tustison_2010} and skull-stripped using ANTs \cite{Avants_2008}. Nonlinear spatial normalization to the ICBM 152 Nonlinear Asymmetrical template version 2009c \cite{Fonov_2009} was performed using ANTs. Brain tissue segmentation cerebrospinal fluid (CSF), white matter, and gray matter was  was performed using FSL's FAST \cite{Zhang_2001}. Functional images were slice timing corrected using AFNI's 3dTshift \cite{Cox_1996} and corrected for head motion using FSL's MCFLIRT \cite{jenkinson2002improved}. "Fieldmap-less" distortion correction was performed by  co-registering each subject's functional image to that subject's intensity-inverted T1-weighted image \cite{wang2017evaluation} constrained with an average field map template \cite{treiber2016characterization}. This was followed by co-registration to the corresponding T1-weighted image using FreeSurfer's boundary-based registration \cite{greve2009accurate} with 9 degrees of freedom. Motion correcting transformations, field distortion correcting warp, BOLD-to-T1 transformation and T1-to-template (MNI) warp were concatenated and applied in a single step with Lanczos interpolation using ANTs. Physiological noise regressors were extracted applying aCompCor \cite{behzadi2007component}. Six principal component time series were calculated within the intersection of the subcortical mask and the union of CSF and WM masks calculated in T1w space, after their projection to the native space of each functional run. Framewise displacement \cite{power2014methods} was calculated for each functional run. Functional images were downsampled to 3 mm resolution. Nuisance variables comprising six head motion parameters (and their derivatives), framewise displacement, linear and quadratic trends, sine/cosine bases for high-pass filtering (0.007 Hz cutoff), and six principal component time series from an anatomically-defined mask of cerebrospinal fluid (CSF) and white matter were regressed out of the signal using AFNI’s 3dTproject \cite{Cox_1996}. Functional response time series were z-scored for each voxel.
%
%Using FMRI (Functional Magnetic Resonance Imaging), blood-oxygen-level dependent(BOLD) temporal fluctuations, \dimension{\FMRI}{\FMRIdim} within each brain is recorded, where \xC \todo{what is C here? is this necessary?}is $1$ and represents the number of channels, \FMRIspaD represents the spacial dimensions of the data and is dependent on the spacial resolution, 2mm or 3mm voxels, of the data collection. \T represents the number of samples taken while the duration of the audio story. The FMRI imaging is done with 1.5 seconds of sampling rate for all data collection. Classifier \FMRIclassifier gives the ground truth of audio dataset the brain imaging data is from.
%
\subsection{Implementation Details}
%
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.6\textwidth]{images/arch_fMRI.pdf}
    \caption{Network architecture for fMRI.}
    \label{fig:arch_fmri}
\end{figure*}
%
We study listener–-listener coupling, where $X$ and $Z$ are a pair of synchronized window of $L=10$ TRs (15 seconds) with voxels selected using (ISC, dDMN, GM) listening to the same story. The neural network $T_\theta(X,Z)$ is illustrated in Figure~\ref{fig:arch_fmri}. It consists of two residual CNN encoders and a distance function. The residual CNN encoders first projects each frame of \xV voxels independently into a $h=256$-dimensional vector. Subsequently 3 blocks of 1D residual convolution layers over the time dimension refines the representation. The distance function takes the $h\times L$ representation of $X$ and $Z$, computes their cosine distance, and passes it through a parameterized scaling layer $M\times \tanh(w* \cos<embed(X),embed(Z)>+b)$, where $w$ and $b$ are parameters.

For \basealgo we use $M=5$, learning rate $\eta=1\times 10^{-3}$, batch size 8192 over 20 iterations. For \metaalgo we use $M=5$, learning rate $\eta=1\times 10^{-3}$, batch size 128 over 80 iterations, meta learning rate $\eta_{\text{meta}}=3\times 10^{-4}$, with BPTT-based meta-optimization over 5000 iterations. For \basealgo we report results on ISC, dDMN and GM masks. For \metaalgo we report results on ISC and dDMN masks, while GM does not fit into the GPU memory due to the high memory consumption of BPTT.
%
%The scoring function $T(x,z)$ takes in features $\phi(\cdot)$ for $x$ $f and  clips, $$(x,zz)=<\phi(x),\phi(z)>$. For each 50-frame $X$ and $Z$, we run a sliding window of 6 frames, compute the 5 frame-differences, and run a 2-layer 1024 LSTM units per layer RNN to encode the 5 1-D frames, and transform the RNN hidden state into a 1024 dimensional vector using 1 linear layer and L2 normalize it. We concatenate those vectors over all sliding windows, resulting in a 1024*45-dimensional representation as $phi(x)$. Effectively, this is running a scoring function for every 6-frame window and average the scores over all windows.. As a baseline we compute for each voxel, the pearson's correlation between that voxel's activations in $X$ and $Z$, and average the pearson's correlation over all voxels as a linear correlation measure between $X$ and $Z$. For 1-D models, we apply either dorsal Default Mode Ntwork (dDMN), Inter Subject Correlation (ISC) or gray matter masks to every frame and string the voxels into a 1-D vector.
%
%\textbf{Pre-processing and Features.}
%
%\textit{Audio and Text.} \change{describe feature vector}
%Different audio segments has been recorded using professional speakers.  Audio -> Text -> Aligned text and audio with timed segments  
%
\subsection{Results}
We study the MI estimation and between-subject time-segment classification of \basealgo and \metaalgo comparing with Pearson's correlation commonly used in ISC analysis.

\noindent\textbf{Quantitative Results.} For the learned $T_\theta(X,Z)$, we use between-subject time-segment classification (BSC) for evaluation \cite{haxby2011common, guntupalli2016model}. Each video is divided into $K$ non-overlapping $L=10 TR$ time segments. The BSC task is 1) one versus one: given a time segment $x$ from an individual, retrieve the corresponding time segment $z$ from another individual out of the $K$ possible segments; 2) one versus rest: retrieve the corresponding time segment $z$ of an individual given a group of time segments ${x}$ excluding that individual. Performance is measured by top-1 retrieval accuracy.

%Quoting Haxby:
%We used a one-nearest neighbor classifier based on vector correlations for BSC [between-subject classification] of 18 s segments of the movie (six time points, TR = 3s). An individual's response vector to a specific time segment was correctly classified if the correlation of that response vector with the group mean response vector (excluding that individual) for the same time segment was higher than all correlations of that vector with group mean response vectors for more than 1,000 other time segments of equal length.
%\red{Figure out how to describe this experiment.  And then perform retrieval: given $x$, retrieve the corresponding $z$ out of the non-overlapping segments. Performance is measured by top-1 retrieval accuracy. In 1 vs 1 setting, $x$ is activation of only 1 subject. In 1 vs rest setting, $x$ is activation of all other subjects. 
For \basealgo, we compute score $T_\theta(X,Z)$ for each pair of $X$ and $Z$ for one versus one, and average over ${X}$ for one versus all. For Pearson correlation, $\rho(X,Z)$ for one vs one, and compute $\rho(\bar{X},Z)$ for one versus all, where $\bar{X}$ is mean of ${X}$ from subjects different than Z.\footnote{Empirically $\rho(\bar{X},Z)$ performs better than $\sum_{X}{\rho(X,Z)}$. For Pearson correlation over multiple voxels, we treat samples from different voxels as i.i.d. samples from a single sequence and compute Pearson correlation. } Results are shown in Tab.~\ref{table:classification}. \basealgo consistently outperforms Pearson correlation on ISC, dDMN and GM for all 4 stories. \metaalgo greatly improves both accuracy and mutual information estimation on the ISC mask. The low performance on dDMN mask is likely due to BPTT optimization unable to decrease the meta learning loss, which could be improved by further improvements on the optimization algorithm.

%
For mutual information estimation, \basealgo predicts 0.637, 0.035 and 0.610 nats of mutual information communicated over $10$ TRs (15 seconds), for ISC, DMN and GM masks respectively.
\input{images/classification.tex}
%
\begin{figure*}[t]
    \centering
    \caption{Top: Top contributing voxels in the learned $T_\theta(X,Z)$ by gradient magnitude $\mathbb{E}_X (\frac{\partial T}{\partial X_i})^2$. Auditory region is highlighted for ISC and GM masks (best in color). Bottom: Evaluation on the "Pie Man" dataset using the ISC mask showing our approach $T_\theta(X,Z)$ versus Pearson correlation over time in the one versus rest case averaged over 20 test subjects.}
    %\includegraphics[width=\textwidth]{images/fig_importance.pdf}
    %\vspace{-13pt}
    %\includegraphics[width=\textwidth]{images/importance_masks_2.pdf}
    \includegraphics[width=\textwidth]{images/importance_masks_3.pdf}
    \label{fig:importance}
    \vspace{-20pt}
\end{figure*}

\noindent\textbf{Qualitative Results.} Fig.~\ref{fig:importance} (top) visualizes voxels that are important to $T(x,z)$ using their gradient magnitude variance for the ISC, dDMN, and GM masks. The models focuses on auditory regions functionally important for perceiving the story stimulus.

Fig.~\ref{fig:importance} (bottom) plots the $T(x,z)$ and intersubject Pearson correlations over time for "Pie Man" using the ISC mask, a sliding window size $L=10$, using the one vs rest scores averaged over all subjects. NeuralMI yields more distinctive peaks.

We identify the peaks in \basealgo for "Pie Man" (with Pearson correlations) over time, then locate the story transcriptions in the $L=10 TRs$ (15 seconds) window corresponding to the peak:
%
\begin{itemize}
    \item 4: ``\ldots toiled for The Ram, uh, Fordham University’s student newspaper. And one day, I’m walking toward the campus center and out comes the elusive Dean McGowen, architect of a policy to replace traditionally \ldots"
    \item 45: "The Dean is covered with cream. So I give him a moment, then I say, `Dean McGowen, would you care to comment on this latest attack?' And he says, `Yes, I would care to comment. \ldots''
    \item 109: "\ldots which makes no sense. Fordham was a Catholic school and we all thought Latin was classy so, that’s what I used. And when I finished my story, I, I raced back to Dwyer and I showed it to him and he read it and he said \ldots"
    \item 122: "Few days later, I get a letter. I opened it up and it says, “Dear Jim, good story. Nice details. If you want to see me again in action, be on the steps of Duane Library \ldots"
    \item 139: "\ldots out comes student body president, Sheila Biel. And now, Sheila Biel was different from the rest of us flannel-shirt wearing, part-time-job working, Fordham students. Sheila was\ldots"
    \item 167: "Pie Man emerged from behind a late night library drop box, made his delivery, and fled away, crying, “Ego sum non una bestia.” And that’s what I reported in my story\ldots"
    \item 213: "\ldots that there was a question about whether she even knew if I existed. So I saw her there and made a mental note to do nothing about it, and then I went to the bar and ordered a drink, and I felt a, a tap on my shoulder. I turned around, and it was her.\ldots"
    \item 239: "And wasn’t I really Pie Man? Hadn’t I brought him into existence? Didn’t she only know about him because of me? But actually \ldots"
    \item 256: "I said, “Yes, Angela, I am Pie Man.' And she looked at me and she said, `Oh, good. I was hoping you’d say that \ldots"
\end{itemize}
We hypothesize that the scripts associated with the peaks may capture points when listeners pay more attention, resulting in the Signal-to-Noise Ratio (SNR) of fMRI scans being enhanced. 
%
%
% (Go to supp)In Figure~\ref{fig:visualization}, we visualize the voxels that contribute the most to $T(X,Z)$ as first order visualization using gradient magnitude. We also visualize pairs of voxels that contributed the most to $T(X,Z)$ as second order visualization using gradient covariance. The average gradient covariance between voxels $Cov(i,j)=Cov(\frac{\partial T}{\partial x_i}$,$\frac{\partial T}{\partial x_j})$. It serves as a proxy to if function of two voxels correlates/decorrelates under the task. Comparing with FC which is next to it, Our approach reveals more high-order non-linear correlations.
%

==> ch/backup.tex <==

\subsection{Dataset and Metrics}
\textbf{New fMRI Dataset.} We apply the proposed model to a newly collected fMRI dataset with 40 participants (mean age = 23.3 years, SD = 8.9, range: 18–53; 27 female) listening to four spoken stories\footnote{Two of the stories were told by a professional storyteller undergoing an fMRI scan; however, fMRI data for the speaker were not analyzed for the present work due to the head motion induced by speech production.}\footnote{The study was conducted in compliance with the Institutional Review Board of the University}. The stories were renditions of “Pie Man” and “Running from the Bronx” by Jim O’Grady \cite{PieMan, Bronx}, “The Man Who Forgot Ray Bradbury” by Neil Gaiman \cite{Forgot}, and “I Knew You Were Black” by Carol Daniel \cite{Black}; story durations were ~7, 9, 14, and 13 minutes, respectively. After scanning, participants completed a questionnaire comprising 25–30 questions per story intended to measure narrative comprehension. The questionnaires included multiple choice, True/False, and fill-in-the-blank questions, as well as four additional subjective ratings per story. Functional and structural images were acquired using a 3T Siemens Prisma with a 64-channel head coil\footnote{See Appendix for additional image acquisition details.}. Briefly, functional images were acquired in an interleaved fashion using gradient-echo echo-planar imaging with a multiband acceleration factor of 3 (TR/TE = 1500/31 ms, resolution = 2.5 mm isotropic voxels, full brain coverage).
%
%In the end, we have 4 stories, each with N=40 fMRI sequences.
%
%The fMRI voxels are mapped onto a standard brain using some technique.
%
%The fMRI sequences are preprocessed into 3mm  voxels.
%
%We normalize the fMRI sequences by mean-std.
%
%We partition data by subject, where sequences from 20 subjects go into train and sequences from the other 20 subjects go into test. 
%
%We focus on the dDMN region, the ISC voxels and the gray matter region.
%
%We also investigate ISC voxels and gray matter with the auditory regions removed for analyzing synchronous non-auditory brain activities.
%
All fMRI data were formatted according to the Brain Imaging Data Structure (BIDS) standard \cite{gorgolewski2016brain} and preprocessed using fMRIPrep \cite{Esteban_2018}\footnote{See Appendix for additional preprocessing details.}. Functional data were corrected for slice timing, head motion, and susceptibility distortion, and normalized to MNI space using nonlinear registration. Nuisance variables comprising head motion parameters, framewise displacement, linear and quadratic trends, sine/cosine bases for high-pass filtering (0.007 Hz), and six principal component time series from cerebrospinal fluid (CSF) and white matter were regressed out of the signal using AFNI \cite{Cox_1996}.

The fMRI data were first partitioned into a seen set of 20 subjects and a unseen set of 20 separate subjects. We restricted our analysis to three subsets of voxels: an anatomically defined gray matter mask (GM; 22,541 voxels), as well as functionally-defined masks of high ISC voxels (ISC; 15,041 voxels) and dorsal Default-Mode Network voxels (dDMN; 3,940 voxels). All masks were defined in MNI space, and the ISC and dDMN masks were defined using independent data from previous studies \cite{simony2016dynamic}.
%The fMRI data comprise \dimension{\FMRI}{\FMRIdim}\todo{what is C here? is this necessary?}\todo{C is left over from our spacial model indicating # of channels.} for each subject, where \FMRIspaD represents the spatial dimensions of each volume and \T represents the number of samples (TRs) during auditory stimulus presentation.
The fMRI data comprise \dimension{\FMRI}{\FMRIdimFlat} for each subject, where \xV represents the flattened and masked voxel space and \T represents the number of samples (TRs) during auditory stimulus presentation.

%For each audio segment, subjects were asked to pay attention and passively listen to the story. Subjects were also instructed to attend to the details of the narrative.


\textbf{Additional Details on Dataset Collection}
Functional and structural images were acquired using a 3T Siemens Magnetom Prisma with a 64-channel head coil. Functional, blood-oxygenation-level-dependent (BOLD) images were acquired in an interleaved fashion using gradient-echo echo-planar imaging with pre-scan normalization, fat suppression, a multiband acceleration factor of 3, and no in-plane acceleration: TR/TE = 1500/31 ms, flip angle = 67°, bandwidth = 2480 Hz/Px, resolution = 2.5 mm3 isotropic voxels, matrix size = 96 x 96, FoV = 240 x 240 mm, 48 axial slices with roughly full brain coverage and no gap, anterior–posterior phase encoding. At the beginning of each scanning session, a T1-weighted structural scan was acquired using a high-resolution single-shot MPRAGE sequence with an in-plane acceleration factor of 2 using GRAPPA: TR/TE/TI = 2530/3.3/1100 ms, flip angle = 7°, resolution = 1.0 x 1.0 x 1.0 mm voxels, matrix size = 256 x 256, FoV = 256 x 256 x 176 mm, 176 sagittal slices, ascending acquisition, anterior–posterior phase encoding, no fat suppression, 5 min 53 s total acquisition time. At the end of each scanning session a T2-weighted structural scan was acquired using the same acquisition parameters and geometry as the T1-weighted structural image: TR/TE = 3200/428 ms, 4 min 40 s total acquisition time. A field map was acquired at the beginning of each scanning session, but was not used in subsequent analyses.

\textbf{Additional Details on Dataset Preprocessing}
Preprocessing was performed using fMRIPrep \cite{Esteban_2018}, a Nipype \cite{Gorgolewski_2011} based tool. T1-weighted images were corrected for intensity non-uniformity using N4 bias field correction \cite{Tustison_2010} and skull-stripped using ANTs \cite{Avants_2008}. Nonlinear spatial normalization to the ICBM 152 Nonlinear Asymmetrical template version 2009c \cite{Fonov_2009} was performed using ANTs. Brain tissue segmentation cerebrospinal fluid (CSF), white matter, and gray matter was  was performed using FSL's FAST \cite{Zhang_2001}. Functional images were slice timing corrected using AFNI's 3dTshift \cite{Cox_1996} and corrected for head motion using FSL's MCFLIRT \cite{jenkinson2002improved}. "Fieldmap-less" distortion correction was performed by  co-registering each subject's functional image to that subject's intensity-inverted T1-weighted image \cite{wang2017evaluation} constrained with an average field map template \cite{treiber2016characterization}. This was followed by co-registration to the corresponding T1-weighted image using FreeSurfer's boundary-based registration \cite{greve2009accurate} with 9 degrees of freedom. Motion correcting transformations, field distortion correcting warp, BOLD-to-T1 transformation and T1-to-template (MNI) warp were concatenated and applied in a single step with Lanczos interpolation using ANTs. Physiological noise regressors were extracted applying aCompCor \cite{behzadi2007component}. Six principal component time series were calculated within the intersection of the subcortical mask and the union of CSF and WM masks calculated in T1w space, after their projection to the native space of each functional run. Framewise displacement \cite{power2014methods} was calculated for each functional run. Functional images were downsampled to 3 mm resolution. Nuisance variables comprising six head motion parameters (and their derivatives), framewise displacement, linear and quadratic trends, sine/cosine bases for high-pass filtering (0.007 Hz cutoff), and six principal component time series from an anatomically-defined mask of cerebrospinal fluid (CSF) and white matter were regressed out of the signal using AFNI’s 3dTproject \cite{Cox_1996}. Functional response time series were z-scored for each voxel.


%Using FMRI (Functional Magnetic Resonance Imaging), blood-oxygen-level dependent(BOLD) temporal fluctuations, \dimension{\FMRI}{\FMRIdim} within each brain is recorded, where \xC \todo{what is C here? is this necessary?}is $1$ and represents the number of channels, \FMRIspaD represents the spacial dimensions of the data and is dependent on the spacial resolution, 2mm or 3mm voxels, of the data collection. \T represents the number of samples taken while the duration of the audio story. The FMRI imaging is done with 1.5 seconds of sampling rate for all data collection. Classifier \FMRIclassifier gives the ground truth of audio dataset the brain imaging data is from.

\subsection{Implementation Details}


\begin{figure*}[t] 
    \centering
    \includegraphics[width=\linewidth]{images/fig_arch.pdf}
    \caption{Network architectures of $T(x,z)$. $T(x,z)$ encodes fMRI activation sequences $x$ and $z$ using a siamese CNN as the embedding network. $T(x,z)$ is computed as a scaled and clamped cosine similarity between the embeddings of $x$ and $z$ using the distance network.}
    \label{fig:arch}
\end{figure*}

\begin{figure*}[t] %sideways
    \centering
    \includegraphics[width=\linewidth]{images/fig_importance2.pdf}
    \caption{Top 100 most important voxels in $T(x,y)$ by gradient variance $\mathbb{E}_X (\frac{\partial T}{\partial x_i})^2$, compared to top 100 voxels with greatest intersubject Pearson correlation $\rho(x_i,z_i)$, for ISC, dDMN, and GM masks.}
    \label{fig:importance2}
\end{figure*}

We study listener–listener coupling, where $x$ and $z$ are a pair of synchronized window of $L=10$ TRs (15 seconds) with voxels selected using (ISC, dDMN, GM) listening to the same story. The scoring function $T(x,z)$ consists of a residual CNN encoder and a distance function. The residual CNN encoder first independently projects each frame of \xV voxels into a $h=256$-dimensional vector. A subsequent 6-layer 1D residual CNN over the time dimension refines the representation. The distance function takes the $h\times L$ representation of $x$ and $z$, computes their cosine distance, and passes it through a parameterized scaling layer\footnote{The scaling layer $f(x,z) = 5\times \tanh( \exp^{w}* \cos<embed(x),embed(z)>+b)$, $w$ and $b$ are parameters.}. We learn the model parameters by maximizing the MINE-f lower-bound using the Adam optimizer with learning rate $1\times 10^{-3}$ and batch size 8192 over 20 iterations.

%The scoring function $T(x,z)$ takes in features $\phi(\cdot)$ for $x$ $f and  clips, $$(x,zz)=<\phi(x),\phi(z)>$. For each 50-frame $X$ and $Z$, we run a sliding window of 6 frames, compute the 5 frame-differences, and run a 2-layer 1024 LSTM units per layer RNN to encode the 5 1-D frames, and transform the RNN hidden state into a 1024 dimensional vector using 1 linear layer and L2 normalize it. We concatenate those vectors over all sliding windows, resulting in a 1024*45-dimensional representation as $phi(x)$. Effectively, this is running a scoring function for every 6-frame window and average the scores over all windows.. As a baseline we compute for each voxel, the pearson's correlation between that voxel's activations in $X$ and $Z$, and average the pearson's correlation over all voxels as a linear correlation measure between $X$ and $Z$. For 1-D models, we apply either dorsal Default Mode Ntwork (dDMN), Inter Subject Correlation (ISC) or gray matter masks to every frame and string the voxels into a 1-D vector.

%\textbf{Pre-processing and Features.}

%\textit{Audio and Text.} \change{describe feature vector}
%Different audio segments has been recorded using professional speakers.  Audio -> Text -> Aligned text and audio with timed segments  


\subsection{Between-subject time-segment classification}

\textbf{Quantitative Results.} For the learned $T(x,z)$, we use between-subject time-segment classification (BSC) for evaluation \cite{haxby2011common, guntupalli2016model}. Each video is divided into $K$ non-overlapping $L=10 TR$ time segments. The BSC task is 1) one versus one: given a time segment $x$ from an individual, retrieve the corresponding time segment $z$ from another individual out of the $K$ possible segments; 2) one versus rest: retrieve the corresponding time segment $z$ of an individual given a group of time segments ${x}$ excluding that individual. Performance is measured by top-1 retrieval accuracy.
%
%Quoting Haxby:
%We used a one-nearest neighbor classifier based on vector correlations for BSC [between-subject classification] of 18 s segments of the movie (six time points, TR = 3s). An individual's response vector to a specific time segment was correctly classified if the correlation of that response vector with the group mean response vector (excluding that individual) for the same time segment was higher than all correlations of that vector with group mean response vectors for more than 1,000 other time segments of equal length.
%\red{Figure out how to describe this experiment.  And then perform retrieval: given $x$, retrieve the corresponding $z$ out of the non-overlapping segments. Performance is measured by top-1 retrieval accuracy. In 1 vs 1 setting, $x$ is activation of only 1 subject. In 1 vs rest setting, $x$ is activation of all other subjects. 
For NeuralMI, we compute score $T(x,z)$ for each pair of $x$ and $z$ for one versus one, and average over ${x}$ for one versus all. For Pearson correlation, $\rho(x,z)$ for one vs one, and compute $\rho(\bar{x},z)$ for one versus all, where $\bar{x}$ is mean of ${x}$.\footnote{Empirically $\rho(\bar{x},z)$ performs better than $\sum_{x}{\rho(x,z)}$. For Pearson correlation over multiple voxels, we treat samples from different voxels as i.i.d. samples from a single sequence and compute Pearson correlation. } Results are shown in Tab.~\ref{table:classification}. Our approach consistently outperforms Pearson correlation by large margins on ISC, dDMN, and GM for all 4 stories. 
%
For mutual information estimation, our model predicts 0.60, 0.04, 0.61 nats of mutual information communicated over $10$ TRs (15 seconds), for ISC, DMN and GM masks respectively.
\input{images/classification.tex}

\begin{figure*}[t]
    \centering
    \caption{Top: Top contributing voxels in the learned $T(x,z)$ by gradient magnitude $\mathbb{E}_X (\frac{\partial T}{\partial x_i})^2$. Auditory region is highlighted for ISC and GM masks (best in color). Bottom: Evaluation on the "Pie Man" dataset using the ISC mask showing our approach $T(x,z)$ versus Pearson correlation over time in the one versus rest case averaged over 20 test subjects.}
    %\includegraphics[width=\textwidth]{images/fig_importance.pdf}
    %\vspace{-13pt}
    %\includegraphics[width=\textwidth]{images/importance_masks_2.pdf}
    \includegraphics[width=\textwidth]{images/importance_masks_3.pdf}
    \label{fig:importance}
    \vspace{-20pt}
\end{figure*}


In Figure~\ref{fig:importance}(bottom), we identify the peaks in NeuralMI for "Pie Man" (with Pearson correlations) over time, then locate the story transcriptions in the $L=10 TRs$ (15 seconds) window corresponding to the peak:
\begin{itemize}
    \item 4: ``\ldots toiled for The Ram, uh, Fordham University’s student newspaper. And one day, I’m walking toward the campus center and out comes the elusive Dean McGowen, architect of a policy to replace traditionally \ldots"
    \item 45: "The Dean is covered with cream. So I give him a moment, then I say, `Dean McGowen, would you care to comment on this latest attack?' And he says, `Yes, I would care to comment. \ldots''
    \item 109: "\ldots which makes no sense. Fordham was a Catholic school and we all thought Latin was classy so, that’s what I used. And when I finished my story, I, I raced back to Dwyer and I showed it to him and he read it and he said \ldots"
    \item 122: "Few days later, I get a letter. I opened it up and it says, “Dear Jim, good story. Nice details. If you want to see me again in action, be on the steps of Duane Library \ldots"
    \item 139: "\ldots out comes student body president, Sheila Biel. And now, Sheila Biel was different from the rest of us flannel-shirt wearing, part-time-job working, Fordham students. Sheila was\ldots"
    \item 167: "Pie Man emerged from behind a late night library drop box, made his delivery, and fled away, crying, “Ego sum non una bestia.” And that’s what I reported in my story\ldots"
    \item 213: "\ldots that there was a question about whether she even knew if I existed. So I saw her there and made a mental note to do nothing about it, and then I went to the bar and ordered a drink, and I felt a, a tap on my shoulder. I turned around, and it was her.\ldots"
    \item 239: "And wasn’t I really Pie Man? Hadn’t I brought him into existence? Didn’t she only know about him because of me? But actually \ldots"
    \item 256: "I said, “Yes, Angela, I am Pie Man.' And she looked at me and she said, `Oh, good. I was hoping you’d say that \ldots"
\end{itemize}
The scripts associated with the peaks may cover important points in the story. 

Figure~\ref{fig:importance2} compares the top 100 most important voxels in $T(x,y)$ with 100 voxels with highest intersubject Pearson correlation. Our approach and the intersubject Pearson correlation generally agree on functionally important voxels. For the ISC and GM masks, our approach seems to show tighter clustering.



\subsection{Connectivity Analysis}

\textbf{Qualitative Results.} Fig.~\ref{fig:importance}(top) visualizes voxels that are important to $T(x,z)$ using their gradient magnitude variance for the ISC, dDMN, and GM masks. The models focuses on auditory regions functionally important for perceiving the story stimulus.
%
% (Go to supp)In Figure~\ref{fig:visualization}, we visualize the voxels that contribute the most to $T(X,Z)$ as first order visualization using gradient magnitude. We also visualize pairs of voxels that contributed the most to $T(X,Z)$ as second order visualization using gradient covariance. The average gradient covariance between voxels $Cov(i,j)=Cov(\frac{\partial T}{\partial x_i}$,$\frac{\partial T}{\partial x_j})$. It serves as a proxy to if function of two voxels correlates/decorrelates under the task. Comparing with FC which is next to it, Our approach reveals more high-order non-linear correlations.
%
Fig.~\ref{fig:importance}(bottom) plots the $T(x,z)$ and intersubject Pearson correlations over time for "Pie Man" using the ISC mask, a sliding window size $L=10$, using the one vs rest scores averaged over all subjects. NeuralMI yields more distinctive peaks.

==> images/10D_gaussian_rho_0.05.tex <==
\begin{table*}[t] 
\caption{10D Gaussian $\rho=0.05$} 
\centering 
\footnotesize 
\begin{tabular}{l | c c c c } 
\toprule 
Approach & \multicolumn{4}{c}{Number of samples}  \\ 
 & 200 & 600 & 2000 & 6000 \\ 
\midrule 
MI-Kraskov  & 0.027  & 0.032  & 0.030  & 0.032 \\ 
\textit{MINE-f} ES & 0.140 $\pm$ 122.666 & 0.014 $\pm$ 42.738 & 0.024 $\pm$ 38.790 & 0.049 $\pm$ 10.974 \\ 
\basealgo& -0.052 $\pm$ 1.776 & -0.010 $\pm$ 1.026 & -0.001 $\pm$ 0.562 & 0.021 $\pm$ 0.324 \\ 
\metaalgo& 0.000 $\pm$ 1.776 & 0.001 $\pm$ 1.026 & 0.008 $\pm$ 0.562 & 0.025 $\pm$ 0.324 \\ 
\midrule 
Ground Truth & \multicolumn{4}{c}{0.050} \\ 
\bottomrule 
\end{tabular} 
\label{table:10d_gaussian_rho0.05} 
\end{table*} 


==> images/10D_gaussian_rho_0.10.tex <==
\begin{table*}[t] 
\caption{10D Gaussian $\rho=0.10$} 
\centering 
\footnotesize 
\begin{tabular}{l | c c c c } 
\toprule 
Approach & \multicolumn{4}{c}{Number of samples}  \\ 
 & 200 & 600 & 2000 & 6000 \\ 
\midrule 
MI-Kraskov  & 0.054  & 0.086  & 0.102  & 0.110 \\ 
\textit{MINE-f} ES & 0.130 $\pm$ 85.894 & 0.240 $\pm$ 208.455 & 0.202 $\pm$ 27.162 & 0.197 $\pm$ 22.396 \\ 
\basealgo& 0.002 $\pm$ 1.776 & 0.068 $\pm$ 1.026 & 0.126 $\pm$ 0.562 & 0.161 $\pm$ 0.324 \\ 
\metaalgo& 0.028 $\pm$ 1.776 & 0.094 $\pm$ 1.026 & 0.139 $\pm$ 0.562 & 0.154 $\pm$ 0.324 \\ 
\midrule 
Ground Truth & \multicolumn{4}{c}{0.200} \\ 
\bottomrule 
\end{tabular} 
\label{table:10d_gaussian_rho0.10} 
\end{table*} 


==> images/10D_gaussian_rho_0.15.tex <==
\begin{table*}[t] 
\caption{10D Gaussian $\rho=0.15$} 
\centering 
\footnotesize 
\begin{tabular}{l | c c c c } 
\toprule 
Approach & \multicolumn{4}{c}{Number of samples}  \\ 
 & 200 & 600 & 2000 & 6000 \\ 
\midrule 
MI-Kraskov  & 0.124  & 0.180  & 0.218  & 0.240 \\ 
\textit{MINE-f} ES & 0.661 $\pm$ 85.894 & 0.457 $\pm$ 208.455 & 0.470 $\pm$ 13.396 & 0.399 $\pm$ 7.734 \\ 
\basealgo& 0.070 $\pm$ 1.776 & 0.271 $\pm$ 1.026 & 0.326 $\pm$ 0.562 & \textbf{0.381 $\pm$ 0.324} \\ 
\metaalgo& 0.077 $\pm$ 1.776 & 0.279 $\pm$ 1.026 & 0.324 $\pm$ 0.562 & \textbf{0.390 $\pm$ 0.324} \\ 
\midrule 
Ground Truth & \multicolumn{4}{c}{0.450} \\ 
\bottomrule 
\end{tabular} 
\label{table:10d_gaussian_rho0.15} 
\end{table*} 


==> images/10D_gaussian_rho_0.15_0.20.tex <==
\begin{table*}[t] 
\caption{10D Gaussian $\rho$} 
\centering 
\footnotesize 
\begin{tabular}{l | c c c c | c c c c  } 
\toprule 
Approach & \multicolumn{4}{c}{10D Gaussian $\rho=0.15$} & \multicolumn{4}{c}{10D Gaussian $\rho=0.20$}  \\ 
 & 200 & 600 & 2000 & 6000 & 200 & 600 & 2000 & 6000 \\ 
\midrule 
MI-Kraskov  & 0.124  & 0.180  & 0.218  & 0.240  & 0.231  & 0.307  & 0.374  & 0.421 \\ 
\textit{MINE-f} ES & 0.661 $\pm$ 85.894 & 0.457 $\pm$ 208.455 & 0.470 $\pm$ 13.396 & 0.399 $\pm$ 7.734 & 0.822 $\pm$ 85.894 & 0.754 $\pm$ 24.458 & 0.728 $\pm$ 13.396 & 0.724 $\pm$ 7.734 \\ 
\basealgo& 0.070 $\pm$ 1.776 & 0.271 $\pm$ 1.026 & 0.326 $\pm$ 0.562 & \textbf{0.381 $\pm$ 0.324} & 0.329 $\pm$ 1.776 & 0.508 $\pm$ 1.026 & \textbf{0.640 $\pm$ 0.562} & \textbf{0.675 $\pm$ 0.324} \\ 
\metaalgo& 0.077 $\pm$ 1.776 & 0.279 $\pm$ 1.026 & 0.324 $\pm$ 0.562 & \textbf{0.390 $\pm$ 0.324} & 0.326 $\pm$ 1.776 & 0.528 $\pm$ 1.026 & \textbf{0.659 $\pm$ 0.562} & \textbf{0.718 $\pm$ 0.324} \\ 
\midrule 
Ground Truth & \multicolumn{4}{c}{0.450} & \multicolumn{4}{c}{0.800}  \\ 
\bottomrule 
\end{tabular} 
\label{table:10d_gaussian_rho_0.15_0.20} 
\end{table*} 


==> images/10D_gaussian_rho_0.20.tex <==
\begin{table*}[t] 
\caption{10D Gaussian $\rho=0.20$} 
\centering 
\footnotesize 
\begin{tabular}{l | c c c c } 
\toprule 
Approach & \multicolumn{4}{c}{Number of samples}  \\ 
 & 200 & 600 & 2000 & 6000 \\ 
\midrule 
MI-Kraskov  & 0.231  & 0.307  & 0.374  & 0.421 \\ 
\textit{MINE-f} ES & 0.822 $\pm$ 85.894 & 0.754 $\pm$ 24.458 & 0.728 $\pm$ 13.396 & 0.724 $\pm$ 7.734 \\ 
\basealgo& 0.329 $\pm$ 1.776 & 0.508 $\pm$ 1.026 & \textbf{0.640 $\pm$ 0.562} & \textbf{0.675 $\pm$ 0.324} \\ 
\metaalgo& 0.326 $\pm$ 1.776 & 0.528 $\pm$ 1.026 & \textbf{0.659 $\pm$ 0.562} & \textbf{0.718 $\pm$ 0.324} \\ 
\midrule 
Ground Truth & \multicolumn{4}{c}{0.800} \\ 
\bottomrule 
\end{tabular} 
\label{table:10d_gaussian_rho0.20} 
\end{table*} 


==> images/10D_gaussian_rho_0.25.tex <==
\begin{table*}[t] 
\caption{10D Gaussian $\rho$} 
\centering 
\footnotesize 
\begin{tabular}{l | c c c c  } 
\toprule 
Approach & \multicolumn{4}{c}{10D Gaussian $\rho=0.25$}  \\ 
 & 200 & 600 & 2000 & 6000 \\ 
\midrule 
MI-Kraskov  & 0.364  & 0.467  & 0.575  & 0.651 \\ 
\textit{MINE-f} ES & 0.871 $\pm$ 42.363 & 1.194 $\pm$ 49.591 & 1.080 $\pm$ 114.176 & 1.061 $\pm$ 10.974 \\ 
\basealgo& 0.460 $\pm$ 1.776 & 0.835 $\pm$ 1.026 & \textbf{0.996 $\pm$ 0.562} & \textbf{1.005 $\pm$ 0.324} \\ 
\metaalgo& 0.524 $\pm$ 1.776 & 0.860 $\pm$ 1.026 & \textbf{1.042 $\pm$ 0.562} & \textbf{1.029 $\pm$ 0.324} \\ 
\midrule 
Ground Truth & \multicolumn{4}{c}{1.252}  \\ 
\bottomrule 
\end{tabular} 
\label{table:10d_gaussian_rho_0.25} 
\end{table*} 


==> images/10D_gaussian_rho_combined.tex <==
\begin{table*}[t] 
\caption{10D Gaussian $\rho$} 
\centering 
\tabcolsep=0.11cm
\scriptsize 


\begin{tabular}{l | c c c c | c c c c  } 
\toprule 
Approach & \multicolumn{4}{c}{10D Gaussian $\rho=0.05$} & \multicolumn{4}{c}{10D Gaussian $\rho=0.10$}  \\ 
 & 200 & 600 & 2000 & 6000 & 200 & 600 & 2000 & 6000 \\ 
\midrule 
MI-Kraskov  & 0.027  & 0.032  & 0.030  & 0.032  & 0.054  & 0.086  & 0.102  & 0.110 \\ 
\textit{MINE-f} ES & 0.140 $\pm$ 122.666 & 0.014 $\pm$ 42.738 & 0.024 $\pm$ 38.790 & 0.049 $\pm$ 10.974 & 0.130 $\pm$ 85.894 & 0.240 $\pm$ 208.455 & 0.202 $\pm$ 27.162 & 0.197 $\pm$ 22.396 \\ 
\basealgo& -0.052 $\pm$ 1.776 & -0.010 $\pm$ 1.026 & -0.001 $\pm$ 0.562 & 0.021 $\pm$ 0.324 & 0.002 $\pm$ 1.776 & 0.068 $\pm$ 1.026 & 0.126 $\pm$ 0.562 & 0.161 $\pm$ 0.324 \\ 
\metaalgo& 0.000 $\pm$ 1.776 & 0.001 $\pm$ 1.026 & 0.008 $\pm$ 0.562 & 0.025 $\pm$ 0.324 & 0.028 $\pm$ 1.776 & 0.094 $\pm$ 1.026 & 0.139 $\pm$ 0.562 & 0.154 $\pm$ 0.324 \\ 
\midrule 
Ground Truth & \multicolumn{4}{c}{0.050} & \multicolumn{4}{c}{0.200}  \\ 
\bottomrule 
\end{tabular} 


\begin{tabular}{l | c c c c | c c c c  } 
\toprule 
Approach & \multicolumn{4}{c}{10D Gaussian $\rho=0.15$} & \multicolumn{4}{c}{10D Gaussian $\rho=0.20$}  \\ 
 & 200 & 600 & 2000 & 6000 & 200 & 600 & 2000 & 6000 \\ 
\midrule 
MI-Kraskov  & 0.124  & 0.180  & 0.218  & 0.240  & 0.231  & 0.307  & 0.374  & 0.421 \\ 
\textit{MINE-f} ES & 0.661 $\pm$ 85.894 & 0.457 $\pm$ 208.455 & 0.470 $\pm$ 13.396 & 0.399 $\pm$ 7.734 & 0.822 $\pm$ 85.894 & 0.754 $\pm$ 24.458 & 0.728 $\pm$ 13.396 & 0.724 $\pm$ 7.734 \\ 
\basealgo& 0.070 $\pm$ 1.776 & 0.271 $\pm$ 1.026 & 0.326 $\pm$ 0.562 & \textbf{0.381 $\pm$ 0.324} & 0.329 $\pm$ 1.776 & 0.508 $\pm$ 1.026 & \textbf{0.640 $\pm$ 0.562} & \textbf{0.675 $\pm$ 0.324} \\ 
\metaalgo& 0.077 $\pm$ 1.776 & 0.279 $\pm$ 1.026 & 0.324 $\pm$ 0.562 & \textbf{0.390 $\pm$ 0.324} & 0.326 $\pm$ 1.776 & 0.528 $\pm$ 1.026 & \textbf{0.659 $\pm$ 0.562} & \textbf{0.718 $\pm$ 0.324} \\ 
\midrule 
Ground Truth & \multicolumn{4}{c}{0.450} & \multicolumn{4}{c}{0.800}  \\ 
\bottomrule 
\end{tabular} 

\begin{tabular}{l | c c c c  } 
\toprule 
Approach & \multicolumn{4}{c}{10D Gaussian $\rho=0.25$}  \\ 
 & 200 & 600 & 2000 & 6000 \\ 
\midrule 
MI-Kraskov  & 0.364  & 0.467  & 0.575  & 0.651 \\ 
\textit{MINE-f} ES & 0.871 $\pm$ 42.363 & 1.194 $\pm$ 49.591 & 1.080 $\pm$ 114.176 & 1.061 $\pm$ 10.974 \\ 
\basealgo& 0.460 $\pm$ 1.776 & 0.835 $\pm$ 1.026 & \textbf{0.996 $\pm$ 0.562} & \textbf{1.005 $\pm$ 0.324} \\ 
\metaalgo& 0.524 $\pm$ 1.776 & 0.860 $\pm$ 1.026 & \textbf{1.042 $\pm$ 0.562} & \textbf{1.029 $\pm$ 0.324} \\ 
\midrule 
Ground Truth & \multicolumn{4}{c}{1.252}  \\ 
\bottomrule 
\end{tabular} 




\label{table:10d_gaussian_rho_0.05_0.10} 
\end{table*} 


==> images/1D_gaussian_rho_0.0.tex <==
\begin{table*}[t] 
\caption{1D Gaussian $\rho=0.0$} 
\centering 
\footnotesize 
\begin{tabular}{l | c c c } 
\toprule 
Approach & \multicolumn{3}{c}{Number of samples}  \\ 
 & 200 & 600 & 2000 \\ 
\midrule 
MI-Kraskov  & 0.031  & 0.003  & 0.007 \\ 
\textit{MINE-f} ES & 0.017 $\pm$ 60.109 & 0.005 $\pm$ 298.833 & 0.001 $\pm$ 19.008 \\ 
\basealgo& -0.044 $\pm$ 1.776 & -0.008 $\pm$ 1.026 & -0.003 $\pm$ 0.562 \\ 
\metaalgo& -0.115 $\pm$ 1.776 & -0.000 $\pm$ 1.026 & -0.000 $\pm$ 0.562 \\ 
\bottomrule 
\end{tabular} 
\label{table:1d_gaussian_rho0.0} 
\end{table*} 


==> images/1D_gaussian_rho_0.0_0.1.tex <==
\begin{table*}[t] 
\caption{1D Gaussian $\rho$} 
\centering 
\footnotesize 
\begin{tabular}{l | c c c | c c c  } 
\toprule 
Approach & \multicolumn{3}{c}{1D Gaussian $\rho=0.0$} & \multicolumn{3}{c}{1D Gaussian $\rho=0.1$}  \\ 
 & 200 & 600 & 2000 & 200 & 600 & 2000 \\ 
\midrule 
MI-Kraskov  & 0.031  & 0.003  & 0.007  & 0.044  & 0.014  & 0.021 \\ 
\textit{MINE-f} ES & 0.017 $\pm$ 60.109 & 0.005 $\pm$ 298.833 & 0.001 $\pm$ 19.008 & 0.038 $\pm$ 151.356 & 0.019 $\pm$ 49.591 & 0.017 $\pm$ 13.396 \\ 
\basealgo& -0.044 $\pm$ 1.776 & -0.008 $\pm$ 1.026 & -0.003 $\pm$ 0.562 & -0.023 $\pm$ 1.776 & 0.014 $\pm$ 1.026 & 0.018 $\pm$ 0.562 \\ 
\metaalgo& -0.115 $\pm$ 1.776 & -0.000 $\pm$ 1.026 & -0.000 $\pm$ 0.562 & -0.064 $\pm$ 1.776 & 0.021 $\pm$ 1.026 & 0.019 $\pm$ 0.562 \\ 
\midrule 
Ground Truth & \multicolumn{3}{c}{0.000} & \multicolumn{3}{c}{0.020}  \\ 
\bottomrule 
\end{tabular} 
\label{table:1d_gaussian_rho_0.0_0.1} 
\end{table*} 


==> images/1D_gaussian_rho_0.1.tex <==
\begin{table*}[t] 
\caption{1D Gaussian $\rho=0.1$} 
\centering 
\footnotesize 
\begin{tabular}{l | c c c } 
\toprule 
Approach & \multicolumn{3}{c}{Number of samples}  \\ 
 & 200 & 600 & 2000 \\ 
\midrule 
MI-Kraskov  & 0.044  & 0.014  & 0.021 \\ 
\textit{MINE-f} ES & 0.038 $\pm$ 151.356 & 0.019 $\pm$ 49.591 & 0.017 $\pm$ 13.396 \\ 
\basealgo& -0.023 $\pm$ 1.776 & 0.014 $\pm$ 1.026 & 0.018 $\pm$ 0.562 \\ 
\metaalgo& -0.064 $\pm$ 1.776 & 0.021 $\pm$ 1.026 & 0.019 $\pm$ 0.562 \\ 
\bottomrule 
\end{tabular} 
\label{table:1d_gaussian_rho0.1} 
\end{table*} 


==> images/1D_gaussian_rho_0.3.tex <==
\begin{table*}[t] 
\caption{1D Gaussian $\rho=0.3$} 
\centering 
\footnotesize 
\begin{tabular}{l | c c c } 
\toprule 
Approach & \multicolumn{3}{c}{Number of samples}  \\ 
 & 200 & 600 & 2000 \\ 
\midrule 
MI-Kraskov  & 0.207  & 0.174  & 0.183 \\ 
\textit{MINE-f} ES & 0.171 $\pm$ 42.363 & 0.172 $\pm$ 42.738 & 0.172 $\pm$ 13.396 \\ 
\basealgo& 0.161 $\pm$ 1.776 & 0.168 $\pm$ 1.026 & 0.175 $\pm$ 0.562 \\ 
\metaalgo& 0.144 $\pm$ 1.776 & 0.176 $\pm$ 1.026 & 0.179 $\pm$ 0.562 \\ 
\bottomrule 
\end{tabular} 
\label{table:1d_gaussian_rho0.3} 
\end{table*} 


==> images/1D_gaussian_rho_0.3_0.5.tex <==
\begin{table*}[t] 
\caption{1D Gaussian $\rho$} 
\centering 
\footnotesize 
\begin{tabular}{l | c c c | c c c  } 
\toprule 
Approach & \multicolumn{3}{c}{1D Gaussian $\rho=0.3$} & \multicolumn{3}{c}{1D Gaussian $\rho=0.5$}  \\ 
 & 200 & 600 & 2000 & 200 & 600 & 2000 \\ 
\midrule 
MI-Kraskov  & 0.207  & 0.174  & 0.183  & 0.533  & 0.510  & 0.513 \\ 
\textit{MINE-f} ES & 0.171 $\pm$ 42.363 & 0.172 $\pm$ 42.738 & 0.172 $\pm$ 13.396 & 0.492 $\pm$ 517.595 & 0.413 $\pm$ 49.591 & 0.492 $\pm$ 38.790 \\ 
\basealgo& 0.161 $\pm$ 1.776 & 0.168 $\pm$ 1.026 & 0.175 $\pm$ 0.562 & 0.423 $\pm$ 1.776 & 0.435 $\pm$ 1.026 & 0.493 $\pm$ 0.562 \\ 
\metaalgo& 0.144 $\pm$ 1.776 & 0.176 $\pm$ 1.026 & 0.179 $\pm$ 0.562 & 0.436 $\pm$ 1.776 & 0.470 $\pm$ 1.026 & 0.494 $\pm$ 0.562 \\ 
\midrule 
Ground Truth & \multicolumn{3}{c}{0.180} & \multicolumn{3}{c}{0.511}  \\ 
\bottomrule 
\end{tabular} 
\label{table:1d_gaussian_rho_0.3_0.5} 
\end{table*} 


==> images/1D_gaussian_rho_0.5.tex <==
\begin{table*}[t] 
\caption{1D Gaussian $\rho=0.5$} 
\centering 
\footnotesize 
\begin{tabular}{l | c c c } 
\toprule 
Approach & \multicolumn{3}{c}{Number of samples}  \\ 
 & 200 & 600 & 2000 \\ 
\midrule 
MI-Kraskov  & 0.533  & 0.510  & 0.513 \\ 
\textit{MINE-f} ES & 0.492 $\pm$ 517.595 & 0.413 $\pm$ 49.591 & 0.492 $\pm$ 38.790 \\ 
\basealgo& 0.423 $\pm$ 1.776 & 0.435 $\pm$ 1.026 & 0.493 $\pm$ 0.562 \\ 
\metaalgo& 0.436 $\pm$ 1.776 & 0.470 $\pm$ 1.026 & 0.494 $\pm$ 0.562 \\ 
\bottomrule 
\end{tabular} 
\label{table:1d_gaussian_rho0.5} 
\end{table*} 


==> images/1D_gaussian_rho_0.7.tex <==
\begin{table*}[t] 
\caption{1D Gaussian $\rho$} 
\centering 
\footnotesize 
\begin{tabular}{l | c c c  } 
\toprule 
Approach & \multicolumn{3}{c}{1D Gaussian $\rho=0.7$}  \\ 
 & 200 & 600 & 2000 \\ 
\midrule 
MI-Kraskov  & 1.080  & 1.077  & 1.078 \\ 
\textit{MINE-f} ES & 1.035 $\pm$ 42.363 & 1.020 $\pm$ 42.738 & 1.015 $\pm$ 114.176 \\ 
\basealgo& 0.947 $\pm$ 1.776 & 0.994 $\pm$ 1.026 & \textbf{1.015 $\pm$ 0.562} \\ 
\metaalgo& 0.944 $\pm$ 1.776 & 0.997 $\pm$ 1.026 & \textbf{1.014 $\pm$ 0.562}\\ 
\midrule 
Ground Truth & \multicolumn{3}{c}{1.072}  \\ 
\bottomrule 
\end{tabular} 
\label{table:1d_gaussian_rho_0.7} 
\end{table*} 


==> images/1D_gaussian_rho_combined.tex <==
\begin{table*}[t] 
\caption{1D Gaussian results} 
\centering 
\footnotesize 



\begin{tabular}{l | c c c | c c c  } 
\toprule 
Approach & \multicolumn{3}{c}{1D Gaussian $\rho=0.0$} & \multicolumn{3}{c}{1D Gaussian $\rho=0.1$}  \\ 
 & 200 & 600 & 2000 & 200 & 600 & 2000 \\ 
\midrule 
MI-Kraskov  & 0.031  & 0.003  & 0.007  & 0.044  & 0.014  & 0.021 \\ 
\textit{MINE-f} ES & 0.017 $\pm$ 60.109 & 0.005 $\pm$ 298.833 & 0.001 $\pm$ 19.008 & 0.038 $\pm$ 151.356 & 0.019 $\pm$ 49.591 & 0.017 $\pm$ 13.396 \\ 
\basealgo& -0.044 $\pm$ 1.776 & -0.008 $\pm$ 1.026 & -0.003 $\pm$ 0.562 & -0.023 $\pm$ 1.776 & 0.014 $\pm$ 1.026 & 0.018 $\pm$ 0.562 \\ 
\metaalgo& -0.115 $\pm$ 1.776 & -0.000 $\pm$ 1.026 & -0.000 $\pm$ 0.562 & -0.064 $\pm$ 1.776 & 0.021 $\pm$ 1.026 & 0.019 $\pm$ 0.562 \\ 
\midrule 
Ground Truth & \multicolumn{3}{c}{0.000} & \multicolumn{3}{c}{0.020}  \\ 
\bottomrule 
\end{tabular} 



\begin{tabular}{l | c c c | c c c  } 
\toprule 
Approach & \multicolumn{3}{c}{1D Gaussian $\rho=0.3$} & \multicolumn{3}{c}{1D Gaussian $\rho=0.5$}  \\ 
 & 200 & 600 & 2000 & 200 & 600 & 2000 \\ 
\midrule 
MI-Kraskov  & 0.207  & 0.174  & 0.183  & 0.533  & 0.510  & 0.513 \\ 
\textit{MINE-f} ES & 0.171 $\pm$ 42.363 & 0.172 $\pm$ 42.738 & 0.172 $\pm$ 13.396 & 0.492 $\pm$ 517.595 & 0.413 $\pm$ 49.591 & 0.492 $\pm$ 38.790 \\ 
\basealgo& 0.161 $\pm$ 1.776 & 0.168 $\pm$ 1.026 & 0.175 $\pm$ 0.562 & 0.423 $\pm$ 1.776 & 0.435 $\pm$ 1.026 & 0.493 $\pm$ 0.562 \\ 
\metaalgo& 0.144 $\pm$ 1.776 & 0.176 $\pm$ 1.026 & 0.179 $\pm$ 0.562 & 0.436 $\pm$ 1.776 & 0.470 $\pm$ 1.026 & 0.494 $\pm$ 0.562 \\ 
\midrule 
Ground Truth & \multicolumn{3}{c}{0.180} & \multicolumn{3}{c}{0.511}  \\ 
\bottomrule 
\end{tabular} 

\begin{tabular}{l | c c c  } 
\toprule 
Approach & \multicolumn{3}{c}{1D Gaussian $\rho=0.7$}  \\ 
 & 200 & 600 & 2000 \\ 
\midrule 
MI-Kraskov  & 1.080  & 1.077  & 1.078 \\ 
\textit{MINE-f} ES & 1.035 $\pm$ 42.363 & 1.020 $\pm$ 42.738 & 1.015 $\pm$ 114.176 \\ 
\basealgo& 0.947 $\pm$ 1.776 & 0.994 $\pm$ 1.026 & \textbf{1.015 $\pm$ 0.562} \\ 
\metaalgo& 0.944 $\pm$ 1.776 & 0.997 $\pm$ 1.026 & \textbf{1.014 $\pm$ 0.562}\\ 
\midrule 
Ground Truth & \multicolumn{3}{c}{1.072}  \\ 
\bottomrule 
\end{tabular} 




\label{table:1d_gaussian_rho_0.0_0.1} 
\end{table*} 


==> images/All_Gaussians_combined.tex <==
\begin{table}
\caption{Mean and confidence intervals for 1D Gaussian. Statistically significant dependency is marked in bold font.} 
\centering 
\scriptsize 
%
\begin{tabular}{l | c c c | c c c  } 
\toprule 
Approach & \multicolumn{3}{c}{1D Gaussian $\rho=0.0$} & \multicolumn{3}{c}{1D Gaussian $\rho=0.1$}  \\ 
 & 200 & 600 & 2000 & 200 & 600 & 2000 \\ 
\midrule 
MI-Kraskov  & 0.031  & 0.003  & 0.007  & 0.044  & 0.014  & 0.021 \\ 
\textit{MINE-f} ES & 0.017 $\pm$ 60.109 & 0.005 $\pm$ 298.833 & 0.001 $\pm$ 19.008 & 0.038 $\pm$ 151.356 & 0.019 $\pm$ 49.591 & 0.017 $\pm$ 13.396 \\ 
\basealgo& -0.044 $\pm$ 1.776 & -0.008 $\pm$ 1.026 & -0.003 $\pm$ 0.562 & -0.023 $\pm$ 1.776 & 0.014 $\pm$ 1.026 & 0.018 $\pm$ 0.562 \\ 
\metaalgo& -0.115 $\pm$ 1.776 & -0.000 $\pm$ 1.026 & -0.000 $\pm$ 0.562 & -0.064 $\pm$ 1.776 & 0.021 $\pm$ 1.026 & 0.019 $\pm$ 0.562 \\ 
\midrule 
Ground Truth & \multicolumn{3}{c}{0.000} & \multicolumn{3}{c}{0.020}  \\ 
\bottomrule 
\end{tabular} 
%
\begin{tabular}{l | c c c | c c c  } 
\toprule 
Approach & \multicolumn{3}{c}{1D Gaussian $\rho=0.3$} & \multicolumn{3}{c}{1D Gaussian $\rho=0.5$}  \\ 
 & 200 & 600 & 2000 & 200 & 600 & 2000 \\ 
\midrule 
MI-Kraskov  & 0.207  & 0.174  & 0.183  & 0.533  & 0.510  & 0.513 \\ 
\textit{MINE-f} ES & 0.171 $\pm$ 42.363 & 0.172 $\pm$ 42.738 & 0.172 $\pm$ 13.396 & 0.492 $\pm$ 517.595 & 0.413 $\pm$ 49.591 & 0.492 $\pm$ 38.790 \\ 
\basealgo& 0.161 $\pm$ 1.776 & 0.168 $\pm$ 1.026 & 0.175 $\pm$ 0.562 & 0.423 $\pm$ 1.776 & 0.435 $\pm$ 1.026 & 0.493 $\pm$ 0.562 \\ 
\metaalgo& 0.144 $\pm$ 1.776 & 0.176 $\pm$ 1.026 & 0.179 $\pm$ 0.562 & 0.436 $\pm$ 1.776 & 0.470 $\pm$ 1.026 & 0.494 $\pm$ 0.562 \\ 
\midrule 
Ground Truth & \multicolumn{3}{c}{0.180} & \multicolumn{3}{c}{0.511}  \\ 
\bottomrule 
\end{tabular} 

\begin{tabular}{l | c c c  } 
\toprule 
Approach & \multicolumn{3}{c}{1D Gaussian $\rho=0.7$}  \\ 
 & 200 & 600 & 2000 \\ 
\midrule 
MI-Kraskov  & 1.080  & 1.077  & 1.078 \\ 
\textit{MINE-f} ES & 1.035 $\pm$ 42.363 & 1.020 $\pm$ 42.738 & 1.015 $\pm$ 114.176 \\ 
\basealgo& 0.947 $\pm$ 1.776 & 0.994 $\pm$ 1.026 & \textbf{1.015 $\pm$ 0.562} \\ 
\metaalgo& 0.944 $\pm$ 1.776 & 0.997 $\pm$ 1.026 & \textbf{1.014 $\pm$ 0.562}\\ 
\midrule 
Ground Truth & \multicolumn{3}{c}{1.072}  \\ 
\bottomrule 
\end{tabular} 
%
\label{table:1D_gaussian} 
\end{table} 
%
\begin{table}
\caption{Mean and confidence intervals for 10D Gaussian. Statistically significant dependency is marked in bold font.} 
\centering 
\scriptsize 
\tabcolsep=0.11cm
\scriptsize 
\begin{tabular}{l | c c c c | c c c c  } 
\toprule 
Approach & \multicolumn{4}{c}{10D Gaussian $\rho=0.05$} & \multicolumn{4}{c}{10D Gaussian $\rho=0.10$}  \\ 
 & 200 & 600 & 2000 & 6000 & 200 & 600 & 2000 & 6000 \\ 
\midrule 
MI-Kraskov  & 0.027  & 0.032  & 0.030  & 0.032  & 0.054  & 0.086  & 0.102  & 0.110 \\ 
\textit{MINE-f} ES & 0.140 $\pm$ 122.666 & 0.014 $\pm$ 42.738 & 0.024 $\pm$ 38.790 & 0.049 $\pm$ 10.974 & 0.130 $\pm$ 85.894 & 0.240 $\pm$ 208.455 & 0.202 $\pm$ 27.162 & 0.197 $\pm$ 22.396 \\ 
\basealgo& -0.052 $\pm$ 1.776 & -0.010 $\pm$ 1.026 & -0.001 $\pm$ 0.562 & 0.021 $\pm$ 0.324 & 0.002 $\pm$ 1.776 & 0.068 $\pm$ 1.026 & 0.126 $\pm$ 0.562 & 0.161 $\pm$ 0.324 \\ 
\metaalgo& 0.000 $\pm$ 1.776 & 0.001 $\pm$ 1.026 & 0.008 $\pm$ 0.562 & 0.025 $\pm$ 0.324 & 0.028 $\pm$ 1.776 & 0.094 $\pm$ 1.026 & 0.139 $\pm$ 0.562 & 0.154 $\pm$ 0.324 \\ 
\midrule 
Ground Truth & \multicolumn{4}{c}{0.050} & \multicolumn{4}{c}{0.200}  \\ 
\bottomrule 
\end{tabular} 
%
\begin{tabular}{l | c c c c | c c c c  } 
\toprule 
Approach & \multicolumn{4}{c}{10D Gaussian $\rho=0.15$} & \multicolumn{4}{c}{10D Gaussian $\rho=0.20$}  \\ 
 & 200 & 600 & 2000 & 6000 & 200 & 600 & 2000 & 6000 \\ 
\midrule 
MI-Kraskov  & 0.124  & 0.180  & 0.218  & 0.240  & 0.231  & 0.307  & 0.374  & 0.421 \\ 
\textit{MINE-f} ES & 0.661 $\pm$ 85.894 & 0.457 $\pm$ 208.455 & 0.470 $\pm$ 13.396 & 0.399 $\pm$ 7.734 & 0.822 $\pm$ 85.894 & 0.754 $\pm$ 24.458 & 0.728 $\pm$ 13.396 & 0.724 $\pm$ 7.734 \\ 
\basealgo& 0.070 $\pm$ 1.776 & 0.271 $\pm$ 1.026 & 0.326 $\pm$ 0.562 & \textbf{0.381 $\pm$ 0.324} & 0.329 $\pm$ 1.776 & 0.508 $\pm$ 1.026 & \textbf{0.640 $\pm$ 0.562} & \textbf{0.675 $\pm$ 0.324} \\ 
\metaalgo& 0.077 $\pm$ 1.776 & 0.279 $\pm$ 1.026 & 0.324 $\pm$ 0.562 & \textbf{0.390 $\pm$ 0.324} & 0.326 $\pm$ 1.776 & 0.528 $\pm$ 1.026 & \textbf{0.659 $\pm$ 0.562} & \textbf{0.718 $\pm$ 0.324} \\ 
\midrule 
Ground Truth & \multicolumn{4}{c}{0.450} & \multicolumn{4}{c}{0.800}  \\ 
\bottomrule 
\end{tabular} 
%
\begin{tabular}{l | c c c c  } 
\toprule 
Approach & \multicolumn{4}{c}{10D Gaussian $\rho=0.25$}  \\ 
 & 200 & 600 & 2000 & 6000 \\ 
\midrule 
MI-Kraskov  & 0.364  & 0.467  & 0.575  & 0.651 \\ 
\textit{MINE-f} ES & 0.871 $\pm$ 42.363 & 1.194 $\pm$ 49.591 & 1.080 $\pm$ 114.176 & 1.061 $\pm$ 10.974 \\ 
\basealgo& 0.460 $\pm$ 1.776 & 0.835 $\pm$ 1.026 & \textbf{0.996 $\pm$ 0.562} & \textbf{1.005 $\pm$ 0.324} \\ 
\metaalgo& 0.524 $\pm$ 1.776 & 0.860 $\pm$ 1.026 & \textbf{1.042 $\pm$ 0.562} & \textbf{1.029 $\pm$ 0.324} \\ 
\midrule 
Ground Truth & \multicolumn{4}{c}{1.252}  \\ 
\bottomrule 
\end{tabular} 
\label{table:10D_gaussian} 
\end{table} 

==> images/classification.tex <==
\begin{table*}[t]%[!htbp]
\vspace{-10pt}
\caption{Segment classification accuracy for NeuralMI versus Pearson's correlation in 1 vs 1 and 1 vs rest (averaging over other subjects). Abbreviations: P: Pieman; F: Forgot; Br: Bronx; Bk: Black, MI: Mutual Information.}
\centering
\scriptsize
\begin{tabular}{ l |c c c c | c | c c c c | c | c c c c | c }
\toprule
%\multicolumn{9}{c}{Classification Accuracy}\\
%\midrule
Classification	& \multicolumn{5}{c}{\textbf{ISC Mask}} & \multicolumn{5}{c}{\textbf{dDMN Mask}} & \multicolumn{5}{c}{\textbf{GM Mask}}  \\
Accuracy (\%) & P & F & Br & Bk & MI & P & F & Br & Bk & MI & P & F & Br & Bk & MI \\
\midrule
Chance & 3.7 & 1.8 & 2.6 & 1.9 & N/A & 3.7 & 1.8 & 2.6 & 1.9 & N/A & 3.7 & 1.8 & 2.6 & 1.9 & N/A \\
Pearson's r 1v1 & 11.1 &  6.8 &  9.4 &  9.6 & N/A &  6.5 &  2.7 &  5.1 &  3.8 & N/A &  9.4 &  4.6 &  8.0 &  6.2 & N/A \\
\basealgo 1v1 & \tb{26.3} & 16.7 & 19.9 & 21.9 & 0.637 &  \tb{7.2} &  \tb{3.0} &  \tb{5.6} &  \tb{4.7} & \tb{0.035} & \tb{26.2} & \tb{17.2} & \tb{21.3} & \tb{23.5} & \tb{0.610} \\
\metaalgo 1v1    & 26.2 & \tb{16.8} & \tb{20.8} & \tb{22.7} & \tb{0.752} & 5.8 & 2.9 & 4.9 & 4.1  & 0.031 & - & - & - & - & -\\
\midrule
Pearson's r 1vR & 35.0 & 20.4 & 25.8 & 31.5 & N/A & 14.8 &  6.4 & \tb{11.8} & 9.9 & N/A & 31.3 & 16.8 & 26.6 & 24.2 & N/A \\
\basealgo 1vR    & 42.8 & 28.0 & 32.8 & 35.9 & 0.637 & \tb{16.5} &  \tb{7.9} & 11.6 & \tb{12.0} & \tb{0.035} & \tb{49.8} & \tb{29.6} & \tb{33.9} & \tb{38.1} & \tb{0.610} \\
\metaalgo 1vR  &  \tb{47.2}  & \tb{32.5} & \tb{39.9} & \tb{41.0} & \tb{0.752} & 13.7 & 7.9 & 8.2 & 8.9 & 0.031 & - & - & - & - & - \\
\bottomrule
\end{tabular}
\label{table:classification}
\vspace{-10pt}
\end{table*}


==> images/sine_wave.tex <==
\begin{table}
\caption{Mean and confidence intervals for synthetic sine wave. Statistically significant dependency is marked in bold font.} 
\centering 
\footnotesize 
\begin{tabular}{l | c c | c c } 
\toprule 
 & \multicolumn{2}{c}{Sine wave $a=20$} & \multicolumn{2}{c}{Sine wave $a=30$} \\
Number of samples & 800 & 2000 & 800 & 2000 \\ 
\midrule 
MI-Kraskov  & 0.935  & 1.528  & 0.592  & 1.020 \\ 
\textit{MINE-f} ES & 1.690 $\pm$ 258.797 & 1.811 $\pm$ 202.122 & 0.937 $\pm$ 319.583 & 1.530 $\pm$ 163.678 \\ 
\basealgo& \textbf{1.149 $\pm$ 0.888} & \textbf{1.582 $\pm$ 0.562} & 0.729 $\pm$ 0.888 & \textbf{1.297 $\pm$ 0.562} \\ 
\metaalgo& \textbf{1.529 $\pm$ 0.888} & \textbf{1.793 $\pm$ 0.562} & \textbf{1.240 $\pm$ 0.888} & \textbf{1.426 $\pm$ 0.562} \\ 
\midrule 
Ground Truth (est.) & \multicolumn{2}{c}{2.304} & \multicolumn{2}{c}{2.299} \\ 
\bottomrule 
\end{tabular} 
\label{table:sine_wave} 
\end{table} 
